Persistence K-theory

This paper studies the basic K-theoretic properties of a triangulated persistence category (TPC). This notion was introduced in our earlier papers on triangulation, persistence, and Fukaya categories (arXiv:2304.01785 and arXiv:2104.12258) and it is a type of category that can be viewed as a refinement of a triangulated category in the sense that the morphisms sets of a TPC are persistence modules. We calculate the K-groups in some basic examples and discuss an application to Fukaya categories and to the topology of exact Lagrangian submanifolds. The second version contains some changes in the exposition and the correction of some minor imprecisions.

==> exp-pics <==

% \begin{figure}[h]
%   \includegraphics[scale=0.85]{punctured-disk.pdf} \centering
% \caption{An immersed Lagrangian from a surgery at
%   $y'$.}\label{f:punctured-disk}
% \end{figure}


  \begin{figure}[htbp]
   \begin{center}
     \includegraphics[scale=0.63]{punctured-disk}
%     \includegraphics[width=0.70\textwidth,
%     height=0.3\textheight]{eta-r}
   \end{center}
   \caption{Replacing $\gamma^{\uparrow}$ by a curve
     $\gamma_V^{\uparrow}$ better approximating  the shape of $V$.}
   \label{f:approx}
\end{figure}



==> filtered-fuk.tex <==
\section{Triangulated persistence Fukaya categories}
\label{s:tpfc}

In this section we apply the theory developed in the paper to the case
of Fukaya categories. In particular we will show that the
$K$-theoretic pairing $\kappa$ from~\S\ref{subsec:pairing} carries
geometric information about Lagrangian submanifolds and immersions.

We begin in~\S\ref{sb:faitpc} with a brief algebraic construction that
associate TPC's to filtered $A_{\infty}$-categories. We then outline
in~\S\ref{sb:ffuk} how to construct (under rather restrictive
assumptions) a model of the Fukaya category which is a genuinely
filtered $A_{\infty}$-category. Finally, in~\S\ref{sb:k-lag} we study
the properties of the pairing $\kappa$ in the case of triangulated
persistence Fukaya categories and show that it can distinguish
embeddings from immersions in situations which are not accessible by
the non-filtered theory.




